RWKV-CLIP: A Robust Vision-Language Representation Learner

Contrastive Language-Image Pre-training (CLIP) has significantly improved performance in various vision-language tasks by expanding the dataset with image-text pairs obtained from websites. This paper further explores CLIP from the perspectives of data and model architecture. To address the prevalence of noisy data and enhance the quality of large-scale image-text data crawled from the internet, we introduce a diverse description generation framework that can leverage Large Language Models (LLMs) to synthesize and refine content from web-based texts, synthetic captions, and detection tags. Furthermore, we propose RWKV-CLIP, the first RWKV-driven vision-language representation learning model that combines the effective parallel training of transformers with the efficient inference of RNNs. Comprehensive experiments across various model scales and pre-training datasets demonstrate that RWKV-CLIP is a robust and efficient vision-language representation learner, it achieves state-of-the-art performance in several downstream tasks, including linear probe, zero-shot classification, and zero-shot image-text retrieval. To facilitate future research, the code and pre-trained models are released at https://github.com/deepglint/RWKV-CLIP

==> table/ablation_study_model_structure.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{cc|cc|cc}
    \toprule
     
    \multicolumn{2}{c|}{Image} & \multicolumn{2}{c|}{Text} & Linear Probe & Zero-shot  \\
     RWKV$_{I}$  & CLIP$_{I}$ & RWKV$_{T}$ & CLIP$_{T}$  & Avg & Avg \\ 
    \midrule
    \Checkmark & \XSolidBrush & \XSolidBrush & \Checkmark & 73.6  & 30.9   \\
    \XSolidBrush & \Checkmark & \Checkmark & \XSolidBrush & 71.0  & 41.1   \\
    \Checkmark & \XSolidBrush & \Checkmark & \XSolidBrush & 74.0  & 37.8   \\
    \Checkmark & \XSolidBrush & \Checkmark & \XSolidBrush & 74.0  & 44.3  \\
    \bottomrule
    \end{tabular}
 } 
\caption{Ablation on model structure.}
\label{tab:ablation-text}
\vspace{-5mm}
\end{table}

==> table/linear_prob_data_distribution.tex <==
\begin{table*}[h]
\centering
\resizebox{0.65\linewidth}{!}{
\begin{tabular}{lcccr}
\toprule
\multicolumn{1}{l}{Dataset} & \multicolumn{1}{c}{Classes} & \multicolumn{1}{c}{Train size} & \multicolumn{1}{c}{Test size} & \multicolumn{1}{c}{Evaluation metric} \\
\midrule
Food101                        & 102                             & 75,750                             & 25,250                            & accuracy                                  \\
CIFAR10                        & 10                              & 50,000                             & 10,000                            & accuracy                                  \\
CIFAR100                       & 100                             & 50,000                             & 10,000                            & accuracy                                  \\
Birdsnap                        & 500                             & 42,138                             & 2,149                             & accuracy                                  \\
SUN397                          & 397                             & 19,850                             & 19,850                            & accuracy                                  \\
Cars                   & 196                             & 8,144                              & 8,041                             & accuracy                                  \\
Aircraft                   & 100                             & 6,667                              & 3,333                             & mean per class                            \\
VOC2007                   & 20                             & 5011                             & 4952                             & 11-point mAP                            \\
DTD           & 47                              & 3,760                              & 1,880                             & accuracy                                  \\
Pets                & 37                              & 3,680                              & 3,669                             & mean per class                            \\
Caltech101                     & 101                             & 3,000                              & 5,677                             & mean-per-class                            \\
Flowers                  & 102                             & 2,040                              & 6,149                             & mean per class                            \\
MNIST                  & 10                             & 60,000                              & 10,000                            & accuracy                            \\
STL10                        & 10                             & 5,000                             & 8,000                            & accuracy                                  \\
EuroSAT                         & 10                              & 10,000                             & 5,000                             & accuracy                                  \\
RESISC45            & 45                              & 3,150                              & 25,200                             & accuracy                                  \\
GTSRB            & 43                 &26,640                 &12,630                                                   & accuracy                                  \\
KITTI            & 4                              & 6770                             & 711                             & accuracy                                  \\
Country211            & 211                              & 42,200                             & 21,100                             & accuracy                                  \\
PCAM            & 2                              & 294,912                             & 32,768                             & accuracy                                  \\
UCF101            & 101                              & 9,537                             & 1,794                            & accuracy                                  \\
Kinetics700            & 700                              & 530,779                             & 33,944                            & mean(top1,top5)                                  \\
CLEVR            & 8                              & 2,000                             & 500                            & accuracy                                  \\
Memes            & 2                              & 8,500                             & 500                            & ROC AUC                                  \\
SST2            & 2                              & 7,792                             & 1,821                            & accuracy                                  \\
ImageNet                        & 1000                            & 1,281,167                          & 50,000                            & accuracy                                  \\
\bottomrule
\end{tabular}}
\caption{List of linear probe datasets with the data distribution and evaluation metrics.}
\label{linearprobedatasets}
% \vspace{-4mm}
\end{table*}

==> table/linear_prob_laion_26.tex <==
\begin{table*}[h]
	\centering
	\resizebox{1.0\linewidth}{!}{
        \begin{sc}
		\begin{tabular}{llcccccccccccccccccccccccccccc}
			\toprule
			 & Method              & \shortstack{Pre-train\\ data} & \rotatebox[origin=lb]{90}{\smash{Food101}} & \rotatebox[origin=lb]{90}{\smash{CIFAR10}} & \rotatebox[origin=lb]{90}{\smash{CIFAR100}} & \rotatebox[origin=lb]{90}{\smash{Birdsnap}} & \rotatebox[origin=lb]{90}{\smash{SUN397}} & \rotatebox[origin=lb]{90}{\smash{Cars}} & \rotatebox[origin=lb]{90}{\smash{Aircraft}} & \rotatebox[origin=lb]{90}{\smash{VOC2007}} & \rotatebox[origin=lb]{90}{\smash{DTD}} & \rotatebox[origin=lb]{90}{\smash{Pets}} & \rotatebox[origin=lb]{90}{\smash{Caltech101}} & \rotatebox[origin=lb]{90}{\smash{Flowers}} & \rotatebox[origin=lb]{90}{\smash{MNIST}} & \rotatebox[origin=lb]{90}{\smash{STL10}} & \rotatebox[origin=lb]{90}{\smash{EuroSAT}} & \rotatebox[origin=lb]{90}{\smash{RESISC45}} & \rotatebox[origin=lb]{90}{\smash{GTSRB}} & \rotatebox[origin=lb]{90}{\smash{KITTI}} & \rotatebox[origin=lb]{90}{\smash{Country211}} & \rotatebox[origin=lb]{90}{\smash{PCAM}} & \rotatebox[origin=lb]{90}{\smash{UCF101}} & \rotatebox[origin=lb]{90}{\smash{Kinetics700}} & \rotatebox[origin=lb]{90}{\smash{CLEVR}} & \rotatebox[origin=lb]{90}{\smash{Memes}} & \rotatebox[origin=lb]{90}{\smash{SST2}} &
             \rotatebox[origin=lb]{90}{\smash{ImageNet}} &
             \rotatebox[origin=lb]{90}{\smash{Average}} \\
			

              \midrule  
              & ALIP-ViT B/32     & LAION10M & 71.5 	& 92.2 	& 76.1 	& 36.3 	& 67.3 	& 70.1 	& 41.8 	& 85.3 	& 71.3 	& 74.3 	& 86.9 	& 90.7 	& 98.0 	& 94.6 	& 95.4 	& 84.3 	& 84.1 	& 70.0 	& 12.9 	& 83.4 	& 75.9 	& 46.4 	& 51.0 	& 54.8 	& 56.5 	& 59.6 & 70.4   \\   
              
              & RWKV-CLIP B/32     & LAION10M & 72.7 & 94.7 & 81.4 & 42.3 & 68.3 & 70.3 & 47.9 & 86.5 & 73.6 & 76.6 & 90.0 & 89.4 & 99.0 & 94.6 & 97.0 & 85.6 & 87.0 & 74.9 & 13.8 & 85.1 & 80.8 & 49.3 & 60.6 & 55.4 & 58.3 & 63.7 & 73.0   \\  \hline
                   
              & ALIP-ViT B/16     & LAION10M & 77.2 	& 93.3 	& 77.0 	& 45.1 	& 69.4 	& 77.3 	& 48.6 	& 87.7 	& 74.5 	& 79.0 	& 88.1 	& 93.0 	& 98.3 	& 96.3 	& 96.3 	& 86.4 	& 83.7 	& 72.2 	& 14.2 	& 85.2 	& 80.1 	& 50.1 	& 55.4 	& 55.7 	& 57.3 	& 64.8  & 73.3  \\    

              & RWKV-CLIP B/16    & LAION10M & 78.9 & 95.1 & 81.8 & 50.3 & 72.0 & 76.8 & 50.3 & 89.4 & 75.4 & 79.7 & 91.9 & 91.7 & 99.0 & 96.4 & 96.9 & 87.8 & 87.4 & 75.7 & 15.2 & 85.5 & 83.9 & 53.0 & 61.8 & 55.9 & 60.0 & 68.4 & 75.4 \\ 
              
              \hline            

              & ALIP-ViT B/32  & LAION30M & 76.7 	& 94.0 	& 79.3 	& 44.2 	& 70.6 	& 77.7 	& 48.4 	& 87.6 	& 74.4 	& 80.4 	& 90.0 	& 93.8 	& 98.3 	& 96.3 	& 96.0 	& 86.7 	& 84.7 	& 72.3 	& 15.0 	& 85.0 	& 81.0 	& 50.6 	& 55.6 	& 56.1 	& 59.8 	& 65.0  & 73.8  \\ 

              & RWKV-CLIP B/32 & LAION30M & 76.6 & 95.6 & 82.8 & 46.0 & 71.0 & 77.9 & 50.0 & 88.2 & 74.5 & 78.9 & 91.6 & 92.1 & 99.0 & 96.5 & 97.1 & 86.9 & 87.6 & 78.9 & 15.2 & 85.6 & 83.4 & 51.8 & 61.6 & 58.9 & 58.9 & 67.2 & 75.2  \\  
			\bottomrule
		\end{tabular}
  \end{sc}}
  \caption{Top-1 accuracy(\%) of linear probe on 26 image classification datasets. }
  \label{tab:linear-probe-big-table}
\end{table*}

==> table/parameter_compare.tex <==
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{l|cc|cc|cc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Image} & \multicolumn{2}{c|}{Text} & \multicolumn{2}{c}{Total} \\
        & \small Params(M)  & \small FLOPs(G) & \small Params(M)  & \small FLOPs(G) & \small Params(M)  & \small FLOPs(G)  \\
        \midrule
        \color{dt}\small CLIP-ViT-B/32  & \color{dt} 87.85 & \color{dt} 8.73  & \color{dt} 63.44 & \color{dt} 5.82 & \color{dt} 151.29 & \color{dt} 14.55  \\
        \small RWKV-CLIP-B/32  &  84.21 & 7.91  &  65.35 & 4.93 &  149.56 & 12.84 \\
	\midrule
        \color{dt}\small CLIP-ViT-B/16  & \color{dt} 86.19 & \color{dt} 33.72 &  \color{dt} 63.44 & \color{dt} 5.82 & \color{dt} 149.63 & \color{dt} 39.54 \\
        \small RWKV-CLIP-B/16  & 82.83 & 31.05 &  65.35 & 4.93 & 148.18 & 35.98 \\
	\bottomrule
    \end{tabular}
    }
\caption{Parameters and FLOPs comparison between CLIP and RWKV-CLIP.}
\label{tab:params}
\end{table}


==> table/prompt_zero_shot_classification.tex <==
\begin{table*}
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{llll}
\toprule
\multicolumn{4}{l}{\bf CIFAR 10 \& CIFAR 100} \\
a photo of a \{label\}. &
a blurry photo of a \{label\}. &
a black and white photo of a \{label\}. &
a low contrast photo of a \{label\}. \\
a high contrast photo of a \{label\}. &
a bad photo of a \{label\}. &
a good photo of a \{label\}. &
a photo of a small \{label\}. \\
a photo of a big \{label\}.&
a photo of the \{label\}.&
a blurry photo of the \{label\}.&
a black and white photo of the \{label\}. \\
a low contrast photo of the \{label\}.&
a high contrast photo of the \{label\}.&
a bad photo of the \{label\}.&
a good photo of the \{label\}. \\
a photo of the small \{label\}.&
a photo of the big \{label\}.& & \\
\midrule
\multicolumn{4}{l}{\bf Food101} \\
a photo of \{label\}, a type of food. & & \\
\midrule
\multicolumn{4}{l}{\bf Caltech101} \\
a photo of a \{label\}. &
a painting of a \{label\}. &
a plastic \{label\}. &
a sculpture of a \{label\}. \\
a sketch of a \{label\}. &
a tattoo of a \{label\}. &
a toy \{label\}. &
a rendition of a \{label\}. \\
a embroidered \{label\}. &
a cartoon \{label\}. &
a \{label\} in a video game. &
a plushie \{label\}. \\
a origami \{label\}. &
art of a \{label\}. &
graffiti of a \{label\}. &
a drawing of a \{label\}. \\
a doodle of a \{label\}. &
a photo of the \{label\}. &
a painting of the \{label\}.&
the plastic \{label\}. \\
a sculpture of the \{label\}.&
a sketch of the \{label\}.&
a tattoo of the \{label\}.&
the toy \{label\}. \\
a rendition of the \{label\}.&
the embroidered \{label\}.&
the cartoon \{label\}.&
the \{label\} in a video game. \\
the plushie \{label\}.&
the origami \{label\}.&
art of the \{label\}.&
graffiti of the \{label\}. \\
a drawing of the \{label\}.&
a doodle of the \{label\}.& & \\
\midrule
\multicolumn{4}{l}{\bf Stanford Cars} \\
a photo of a \{label\}.&
a photo of the \{label\}.&
a photo of my \{label\}.&
i love my \{label\}! \\
a photo of my dirty \{label\}.&
a photo of my clean \{label\}.&
a photo of my new \{label\}.&
a photo of my old \{label\}. \\
\midrule
\multicolumn{4}{l}{\bf DTD} \\
a photo of a \{label\} texture.&
a photo of a \{label\} pattern.&
a photo of a \{label\} thing.&
a photo of a \{label\} object. \\
a photo of the \{label\} texture. &
a photo of the \{label\} pattern. &
a photo of the \{label\} thing. &
a photo of the \{label\} object. \\
\midrule
\multicolumn{4}{l}{\bf FGVC Aircraft} \\
a photo of a \{label\}, a type of aircraft.&
a photo of the \{label\}, a type of aircraft.& & \\
\midrule
\multicolumn{4}{l}{\bf Flowers102} \\
a photo of a \{label\}, a type of flower. &&& \\
\midrule
\multicolumn{4}{l}{\bf Pets } \\
a photo of a \{label\}, a type of pet.&&& \\
\midrule
\multicolumn{4}{l}{\bf  SUN39} \\
a photo of a \{label\}.&
a photo of the \{label\}.&& \\
\midrule
\multicolumn{4}{l}{\bf  ImageNet} \\
a bad photo of a \{label\}. & 
a photo of many \{label\}. &
a sculpture of a \{label\}. &
a photo of the hard to see \{label\}. \\
a low resolution photo of the \{label\}. & 
a rendering of a \{label\}. &
graffiti of a \{label\}. &
a bad photo of the \{label\}.  \\
a cropped photo of the \{label\}. &
a tattoo of a \{label\}. & 
the embroidered \{label\}. &
a photo of a hard to see \{label\}.  \\
a bright photo of a \{label\}.&
a photo of a clean \{label\}.&
a photo of a dirty \{label\}.&
a dark photo of the \{label\}. \\
a drawing of a \{label\}.&
a photo of my \{label\}.&
the plastic \{label\}.&
a photo of the cool \{label\}. \\
a close-up photo of a \{label\}.&
a black and white photo of the \{label\}.&
a painting of the \{label\}.&
a painting of a \{label\}. \\
a pixelated photo of the \{label\}.& 
a sculpture of the \{label\}.&
a bright photo of the \{label\}.&
a cropped photo of a \{label\}. \\
a plastic \{label\}.&
a photo of the dirty \{label\}.& 
a jpeg corrupted photo of a \{label\}.&
a blurry photo of the \{label\}. \\
a photo of the \{label\}.&
a good photo of the \{label\}.&
a rendering of the \{label\}.&
a \{label\} in a video game. \\
a photo of one \{label\}.&
a doodle of a \{label\}.&
a close-up photo of the \{label\}.&
a photo of a \{label\}. \\
the origami \{label\}.&
the \{label\} in a video game.&
a sketch of a \{label\}.&
a doodle of the \{label\}. \\
a origami \{label\}.&
a low resolution photo of a \{label\}.&
the toy \{label\}.&
a rendition of the \{label\}. \\
a photo of the clean \{label\}.& 
a photo of a large \{label\}.& 
a rendition of a \{label\}.&
a photo of a nice \{label\}. \\
a photo of a weird \{label\}.& 
a blurry photo of a \{label\}.&
a cartoon \{label\}.&
art of a \{label\}. \\
a sketch of the \{label\}.& 
a embroidered \{label\}.&
a pixelated photo of a \{label\}.&
itap of the \{label\}. \\
a jpeg corrupted photo of the \{label\}.& 
a good photo of a \{label\}.&
a plushie \{label\}.&
a photo of the nice \{label\}. \\
a photo of the small \{label\}.& 
a photo of the weird \{label\}.&
the cartoon \{label\}.&
art of the \{label\}. \\
a drawing of the \{label\}.& 
a photo of the large \{label\}.& 
a black and white photo of a \{label\}.&
the plushie \{label\}. \\
a dark photo of a \{label\}.& 
itap of a \{label\}.& 
graffiti of the \{label\}.& 
a toy \{label\}. \\
itap of my \{label\}.& 
a photo of a cool \{label\}.&
a photo of a small \{label\}.& 
a tattoo of the \{label\}. \\
\bottomrule
\end{tabular}}
\caption{Full list of prompts to evaluate the performance of zero-shot classification on 11 visual recognition datasets.}
\label{tab:prompt}
\end{table*}
